Hide and seek: how PDFs can conceal New Physics

The interpretation of LHC data, and the assessment of possible hints of new physics, require the precise knowledge of the proton structure in terms of parton distribution functions (PDFs). We present a systematic methodology designed to determine whether and how global PDF fits might inadvertently 'fit away' signs of new physics in the high-energy tails of the distributions. We showcase a scenario for the High-Luminosity LHC, in which the PDFs may completely absorb such signs of new physics, thus biasing theoretical predictions and interpretations. We discuss strategies to single out the effects in this scenario, and disentangle the inconsistencies that stem from them. Our study brings to light the synergy between the high luminosity programme at the LHC and future low-energy non-LHC measurements of large-$x$ sea quark distributions. The analysis code used in this work is made public so that any users can test the robustness of the signal associated to a given BSM model against absorption by the PDFs.

==> sec-problem.tex <==
\section{The  impact of LHC data on PDFs}
\label{sec:problem}

As we mentioned in Sect.~1, modern PDF analyses include an increasing
portion of LHC data~\cite{Ball:2021leu,Bailey:2020ooq,Hou:2019efy,Ball:2017nwa,Alekhin:2017kpj}.
In the recent \nnpdf{} analysis~\cite{Ball:2021leu}, which is the
global analysis that we use as a baseline for our study thanks to the
availability of the {\tt NNPDF} public code~\cite{NNPDF:2021uiq}, 
nearly 30\% of the data included in the fit are LHC data. The LHC data not only significantly reduce
PDF uncertainty, but they have a significant pull on the light quarks in the medium and large-$x$ regions,
and a significant although weaker pull in the large-$x$ gluon.  
Such shifts translate into pulls in the large invariant mass region of the \textit{integrated luminosity}. Recall that the integrated luminosity for the parton pair $i,j$ is defined as:
\begin{equation}
\label{eq:integrated_luminosity}
  {\cal L}_{ij}(m_X,\sqrt{s}) = \frac{1}{s}\int\limits_{-y}^{y}\,d\tilde{y}\,f_{i}\left(\frac{m_X}{\sqrt{s}}e^{\tilde{y}},m_X\right)\, \left(\frac{m_X}{\sqrt{s}}e^{-\tilde{y}},m_X\right),
  \end{equation}
 where $f_i \equiv f_i(x,Q)$ is the PDF corresponding to the parton flavour $i \in \{u,d,s,c,b,\bar{u},\bar{d},\bar{s},\bar{c},\bar{b},g\}$, and the integration limits are defined by:
 \begin{equation}
 \label{eq:rapidity}
  y=\ln\left(\frac{\sqrt{s}}{m_X}\right).
  \end{equation}
The pull is largest in the quark-quark and quark-antiquark luminosities, which are defined respectively by:
  \begin{align}
    {\cal L}_{qq}(m_X,\sqrt{s}) &= \sum_{\substack{i,j \in \{u,d,s,c,b \\ \bar{u}, \bar{d}, \bar{s}, \bar{c}, \bar{b}\}}} {\cal L}_{ij}(m_X,\sqrt{s}),\\[1.5ex]
      {\cal L}_{q\bar{q}}(m_X,\sqrt{s}) &= \sum_{i \in \{u,d,s,c,b\}}   {\cal L}_{i\bar{i}}(m_X,\sqrt{s}).
    \end{align}
This is displayed in Fig.~\ref{fig:nnpdf40}, in which the impact of the inclusion of LHC data in the \nnpdf{} analysis is shown.  
\begin{figure}[h!]
	\includegraphics[width=0.49\linewidth]{Figures/NNPDF40_no_lhc.pdf}
	\includegraphics[width=0.49\linewidth]{Figures/NNPDF40_no_lhc_qq.pdf}
	\caption{The impact of the inclusion of LHC data in the \nnpdf analysis, in particular on the $q\bar{q}$ (left panel) and $qq$ (right panel) integrated luminosities, integrated in the central region, $|y|<2.5$ at $\sqrt{s}$ = 14 TeV.}
        \label{fig:nnpdf40}
\end{figure}

Current data reach $m_X\sim 2$ TeV, mostly thanks to the jet and
di-jets double differential distributions in the jet transverse momentum and rapidity~\cite{ATLAS:2017kux,CMS:2016lna,Chatrchyan:2012bja, Aaboud:2017wsi,Khachatryan:2016wdh},
top quark pair invariant mass distributions~\cite{Aaboud:2016iot,CMS:2017iqf,CMS:2018htd,CMS:2018adi,ATLAS:2019hxz, LHCb:2018usb},
high-mass Drell-Yan pair invariant mass~\cite{ATLAS:2013xny,ATLAS:2016gic,ATLAS:2017rue,CMS:2013zfg,CMS:2014jea} and transverse momentum distributions~\cite{Aaboud:2017soa, Aad:2019wmn, CMS:2018mdl,Sirunyan:2017wgx}. As more data of Run II
are delivered in their full luminosity and Run III data are collected and analysed, more and more high energy data from the LHC will be included in PDF analyses.
Several projections studies at the LHC High-Luminosity (HL-LHC) phase~\cite{AbdulKhalek:2018rok} show that there will be enough luminosity to have increased statistics in the $m_X\sim 3-4$ TeV region and in the large-$y$ region, and this
will strongly impact and improve our knowledge of the PDFs at large-$x$. 

The $\gtrsim 1\sigma$ tension between the integrated $q\bar{q}$ parton luminosity obtained by not including
LHC data and the one obtained from a fit which does include the LHC data is a sign of some tension, which might come
from different sources: either a tension between the experimental
data included in a fit, or a tension due to missing higher order
uncertainties that pull theoretical predictions in different
directions, or some hints for new physics in the distributions probing
high energies. 

Global PDF  analyses have a way to determine a {\it maximally consistent} set of data to include in PDF fits, and indeed
various choices on the datasets to be included are made by each PDF fitting collaboration on whether to 
include or not a given dataset, on the basis of the compatibility with the bulk of the dataset included in a
global fit of PDFs. For example in the {\tt CT18} analysis~\cite{Hou:2019efy}, three
alternative fits are delivered on top of the nominal one, the {\tt CT18A},
{\tt CT18X}, and {\tt CT18Z}, the former being the product of adding
the precise ATLAS 7 TeV W/Z data into the {\tt CT18} fit at the cost of
deteriorating the data-theory agreement with other datasets that are
sensitive to the proton's strangeness, the second being a variation
of {\tt CT18} with a different QCD scale for the low-$x$ DIS data;
the latter containing all the above variations.
The differences between the CT18 and CT18Z data sets are
non-negligible in many applications and reflects either a genuine issue with
dealing with data that pull different directions or a lack of 
flexibility in a fitting methodology that is not able to accommodate
many data at the same time.  

The \nnpdf analysis, on the other hand, starts from an extended dataset out of which a maximally
consistent baseline dataset is determined. The latter is determined through a two-step procedure.
First, datasets that are problematic either in terms of fit quality, or because of the
stability properties of their covariance matrix, are flagged.
This is done by comparing for
each measurement respectively the value of the $\chi^2/n_{\rm dat}$, the number of standard deviations $n_\sigma$
by which the value of the $\chi^2$ per data point differs from the expected unit value and finally 
the value of a  covariance matrix stability indicator. 
%The latter is important because, given the high precision of the LHC data, many
%datasets are now limited by systematic, rather than statistical,
%uncertainties. In these situations, the $\chi^2$ of a given
%dataset is extremely sensitive to small differences in the correlation model assumed for the experimental %systematic errors.
%This implies that small inaccuracies in the estimate of the experimental
%correlated systematic uncertainties can potentially induce spurious
%disagreements between theory predictions and experimental data and a poor $\chi^2$ may be caused solely by %an instability
%of the experimental covariance matrix upon its inversion, rather than by
%a genuine tension with the rest of the data in the fit, or by an inaccuracy in
%the theory. 
The procedure does not yield a full understanding of the nature of the inconsistencies, but rather helps singling out and excluding from the baseline dataset inconsistent data based on objective
criteria determined by the given thresholds. 
%
Measurements for which thresholds are exceeded are then subject to a
dedicated weighted fit. The measurement is then retained or discarded
based on the results of this weighted fit.
%
The thresholds in the \nnpdf analysis are given by:
\begin{enumerate}
  \item The total $\chi^2$ per data point. Datasets for
    which $\chi^2> 1.5$ are singled out.
    \item The number of standard deviations $n_\sigma$ by which the value of the
  $\chi^2$ per data point differs from the expected unit value:
  \begin{equation}\label{eq:nsigma}
    n_\sigma\equiv
    \frac{\chi^2-1}{\sigma_{\chi^2}}=\frac{\chi^2-1}{\sqrt{2/n_{\rm dat}}}.
  \end{equation}
  Datasets for which $|n_\sigma|> 2$ are singled out.  
  \item The stability metric $Z$ defined in Ref.~\cite{Kassabov:2022pps}.
Datasets with $Z> 4$ are singled out, on the basis that the induced changes in the resulting covariance matrix are
very likely within the precision to which they were determined.
\end{enumerate}
%
The two relevant estimators for our analysis are 1. and 2. The first estimator flags all situations in which the significance of the discrepancy does not depend on the number of
data points, such as for instance a missing higher order correction
that affects all data points. The second is instead sensitive to
cases in which there might be issues related to systematic
uncertainties and their correlation, whose significance depends on
the number of data points. Datasets are flagged if either 1. and
2. occur at the same time ($\chi^2/n_{\rm dat}>1.5$ and $n_{\sigma}>2$).
%or if 2. and 3. occur at the same time  ($n_{\sigma}>2$ and $Z>4$). 
If a dataset is flagged according to this condition, then a weighted fit is performed, 
{\it i.e.} a fit in which a dataset is given a
larger weight inversely proportional to the number of data-points,
namely
\begin{equation}
\chi^2=\frac{1}{n_{\rm dat}}\,\sum_{i=1}^{n_{\rm dat}} \,n_{\rm
  dat}^{(i)}\,\chi^2_i \qquad \chi^2_w=\frac{1}{n_{\rm dat}-n_{\rm
    dat}^{j}}\,\sum_{i=1,i\neq j}^{n_{\rm exp}} \,n_{\rm
  dat}^{(i)}\,\chi^2_i \, + \,w^{(j)}\chi^2_j,
  \end{equation}
  with
  \begin{equation}
    \label{eq:wgts}
    w^{(j)} = n_{\rm dat}/n_{\rm dat}^{(j)}.
    \end{equation}
If the data-theory agreement improves by setting below thresholds and the
data-theory agreement of the other datasets does not deteriorate in
any statistically relevant way, then the dataset is kept in the
baseline fit, else the dataset is discarded.  If a dataset is flagged according to
the latter condition, then a fit with a regulated covariance matrix is
performed and, if the data-theory agreement improves then the dataset
is kept, else it is discarded. 
%
In our analysis, given that we utilise artificial Monte Carlo data
that have already been scrutinised under the stability of the
covariance matrix, we focus on the first criterion and flag data with
$\chi^2/n_{\rm dat}>1.5$ and $n_{\sigma}>2$ in the various scenarios
that we consider and perform weighted fits to see whether the dataset
should be kept or discarded on the basis of the inconsistency with the
bulk of the other datasets. 

We will see that the latter are a necessary condition to determine a bulk of maximally
consistent datasets, but they are not sufficient, as they still allow
New Physics contamination to go undetected. As a result, we propose a
further criterion to be added to the list above, that prevents this
from happening. The criterion is based on the {\it weighted fit}
methodology and stems from the fact that, if some energy-growing
effect associated to the presence of New Physics in the data shows up in the tails
of the distributions, PDFs might accommodate this effect and absorb it
only up to a point. If the datasets that are affected by New
Physics are given a large weight in the fit, the tension with the
bulk of the datasets that is perfectly described by the SM would eventually show up. Hence by giving a
larger weight to that specific New-Physics-affected dataset, the
disagreement with the bulk of the dataset should become more apparent. Depending on the kind of New Physics
that data might reveal, the effect might affect either of the three
classes of the high energy processes entering PDF fits, namely: (i)
jets and dijets, (ii) top and (iii) Drell-Yan. Our proposed strategy
is highlighted as follows:
\begin{itemize}
\item Perform three weighted fits by giving larger weights (set
  according to Eq.~\eqref{eq:wgts}) to all the
  datasets belonging to each of the process categories highlighted above
  that span an energy range above a given $Q_{\rm max}$ scale. One
  might want to give a larger weight only to the subset of data-points
  that probe a scale $Q>Q_{\rm max}$, however this would neglect the
  correlations among data-points that belong to the same dataset. 
\item If any of the three weighted fits displays incompatibility, as
  with a larger weight its $\chi^2$ improves while deteriorating the $\chi^2$ of other
  datasets, then one should exclude the datasets from the baseline fits.
  \item Rerun the test with a larger and lower values of $Q_{\rm
      max}$, say $Q_{\rm max}/2$ and $2\,Q_{\rm max}$, to assess the stability of the result upon the somewhat arbitrary
    choice of the scale at which New Physics effects are showing. 
  \end{itemize}
In Sect.~5 we will check explicitly the effect and robustness of this
criterion, in the case of contamination that we will identify in the
the rest of the paper. 


==> tables/tab_chi2_w8.tex <==
\begin{table}[t]
        \tiny
        \centering
        \begin{tabular}{lc|c|c|c|c|c|}
                \toprule
       & & \multicolumn{2}{c}{SM} & \multicolumn{2}{c}{$W=8\cdot 10^{-5}$}\\
          \midrule
       Dataset  & $n_{\rm dat}$ & $\chi^2$ &  $n_\sigma$ & $\chi^2$ & $n_\sigma$ \\
          \midrule
 NMC $F^d_2/F^p_2$         & 121 & 0.90 & -0.78 & 0.94 &-0.47 \\
 NMC $\sigma^{\rm NC,p}$ & 204 & 0.93 & -0.71 & 0.93 &-0.71 \\
 SLAC $F^p_2$                   & 33 & 0.52 & -1.95 & 0.55 & -1.83 \\
SLAC $F^d_2$                   & 34 & 1.12 & +0.49 &  1.12 & +0.49 \\
BCDMS $F^p_2$                & 333 & 1.04 & +0.51 &1.03 &+0.39 \\
BCDMS $F^d_2$                & 248 & 0.93 & -0.78 & 0.93 &-0.78 \\
CHORUS $\sigma^\nu_{\rm CC}$ & 416 & 0.98 &-0.28&0.98 &-0.28 \\
CHORUS $\sigma^{\bar\nu}_{\rm CC}$& 416 & 0.95 &-0.72&0.95 &-0.72 \\
NuTeV $\sigma^\nu_{\rm CC}$ (dimuon) & 39 & 0.85 &-0.66& 0.87 &-0.57 \\
NuTeV $\sigma^{\bar\nu}_{\rm CC}$ (dimuon) & 37 & 0.48&-2.23& 0.59&-1.76 \\
                    \midrule
HERA I+II $\sigma^p_{\rm NC} e^-$ & 159 & 1.01&+0.09& 1.02&+0.18 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (460 GeV) & 204 &0.95&-0.51& 0.95&-0.51 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (575 GeV) & 254 &1.12 &+1.35&1.12 &+1.35 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (820 GeV) & 70 &0.89 &-0.65&0.90 &-0.59 \\
HERA I+II $\sigma^p_{\rm NC} e^+$ (920 GeV) & 377 & 0.94&-0.82&0.95 &-0.69 \\
          HERA I+II $\sigma^p_{\rm CC} e^+$ & 42 & 1.22&+1.01&1.22 &+1.01 \\
          HERA I+II $\sigma^p_{\rm CC} e^+$ & 39 & 1.06 &+0.26&1.03 &+0.13\\
          HERA I+II $\sigma^c_{\rm NC}$    & 37 & 0.83 &-0.73&0.84 &-0.69 \\
         HERA I+II $\sigma^b_{\rm NC}$     & 26 & 1.15 &+0.54&1.15&+0.54 \\
                \midrule
                \textbf{Total DIS} & \textbf{3089} & \textbf{0.98} &-0.79&\textbf{0.98} & -0.79 \\
                \midrule
           E886 \(\sigma^p\) (NuSea) & 89 & 1.02&+0.13&0.97 &-0.20 \\
           E886 \(\sigma^{d}/2\sigma^p\) (NuSea) & 15 & 1.17 &+0.46& 1.42&+1.15 \\
           E605 \(\sigma^p\) & 85 & 0.38&-4.04 &0.37 & -4.11\\
           E906 \(\sigma^{d}/2\sigma^p\) (SeaQuest) & 6 & 0.59&-0.71&0.67 &-0.57 \\
          \midrule
           CDF $Z$ differential & 28 & 1.02 &+0.07&1.00 &+0.00\\
           D0  $Z$ differential & 28 & 0.98 &-0.07& 1.00&+0.00\\
           D0  $W$ muon asymmetry & 9 &1.23 &+0.48&1.48 &+1.02\\
                \midrule
         ATLAS low-mass DY 7\,TeV & 6 &1.21 &+0.36&1.21 &+0.36 \\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=35\,{\rm pb}^{-1}$) & 30 & 0.78&-0.85& 0.78&-0.85 \\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) central& 46 & 1.39&+1.87& 1.44&+2.11\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) forward&15 & 0.91&-0.25& 0.92&-0.22 \\
         ATLAS low-mass DY 2D 8 TeV&60 & 0.87&-0.71& 0.86&-0.77 \\
        ATLAS $\sigma^{\rm tot}_{W,Z}$13 TeV & 3 &0.38 &-0.76&0.40&-0.73 \\
        ATLAS $W^+$+jet 8 TeV   &15&1.26&+0.71 &1.24 &+0.66 \\       
        ATLAS $W^-$ +jet 8 TeV   &15&1.02&+0.05 &0.98 &-0.05 \\       

          ATLAS $Z$ $p_T$ 8 TeV $(p_T , m_{ll})$& 44 &0.91 &-0.42&0.91 &-0.42 \\
          ATLAS $Z$ $p_T$ 8 TeV $(p_T , y_Z)$ & 48 &0.70 &-1.47&0.68 &-1.57 \\
                \midrule
CMS $W$ electron asymmetry 7 TeV & 11 &1.48&+1.13&1.50 &+1.17 \\
CMS $W$ muon asymmetry 7 TeV & 11 &1.22 &+0.52&1.28 &+0.66 \\
CMS $W$ rapidity 8 TeV& 22 &1.36 &+1.19& 1.37&+1.23 \\
 CMS  \(Z_{p_T}\) 8 TeV  & 28 &0.83&-0.64&0.82&-0.67\\
                \midrule
LHCb \(Z\rightarrow ee\)  7\,TeV & 9 &0.69&-0.66&0.69&-0.66 \\
LHCb \(W,Z\rightarrow\mu\) 7\,TeV & 29 &0.99&-0.04&0.94&-0.23 \\
LHCb \(Z\rightarrow ee\)  8\,TeV &17  &1.24&+0.70&1.24&+0.70 \\
LHCb \(W,Z\rightarrow\mu\) 8\,TeV &30&0.85&-0.58&0.74&-1.0\\
LHCb \(Z\rightarrow ee\)  13\,TeV & 15 &1.58&+1.59&1.60&+1.64 \\
LHCb \(Z\rightarrow\mu\) 13\,TeV & 16 &1.36&+1.02&1.37&+1.05 \\
                \midrule
                \textbf{Total DY (excl. HM)} & \textbf{670} & \textbf{xx} & \textbf{xx}& & \\
                \midrule
                ATLAS high-mass DY 7 TeV (${\cal L}=49\,{\rm fb}^{-1}$)& 13 &0.40 &-1.53& 0.40&-1.53 \\
                ATLAS high-mass DY 2D 8 TeV & 46 & 0.94&-0.29&0.94&-0.29 \\
                CMS high-mass DY 2D 7 TeV & 117 &0.92&-0.61&0.92&-0.61 \\
                CMS high-mass DY 8 TeV & 41 &1.30 &+1.36&1.29 &+1.31 \\
                CMS high-mass DY 13 TeV & 43 &1.06 &+0.28&1.07 &+0.32 \\
                \midrule
                \textbf{Total DY (HM only)} & \textbf{260} & \textbf{xx} & \textbf{xx}& & \\
                \midrule
%                \textbf{Total (excl. HL-LHC)} & \textbf{4715} & \textbf{xx} & \textbf{xx}& & \\
%                \midrule
                HL-LHC CC \(e\)& 16 & 0.79 &-0.60 & 1.00 & +0.0 \\ %% SM vs  Wcont   | Wcont vs SM
                HL-LHC CC \(\mu\)& 16 & 0.55 & -1.27 & 0.74 & -0.74\\
                HL-LHC NC \(e\)& 12 & 1.63 & +1.54 & 1.61 &+1.49 \\
                HL-LHC NC \(\mu\)& 12 & 0.81 &-0.46 & 0.79 &-0.51  \\
                \midrule
                \textbf{Total HL-LHC only} & \textbf{56} &\textbf{0.92} &-0.42 & \textbf{1.03} &+0.16 \\
                \midrule
                \textbf{Total} & \textbf{4771} & \textbf{0.97} & -1.41 & \textbf{0.96} &-1.89 \\
                \bottomrule
        \end{tabular}
        \caption{Values of the \(\chi^2\) per data point across all datasets
        used in this study. We tabulate values for the baseline PDF set as well
        as those obtained in the contaminated PDF fit. \label{tab:chi2w000008}}
\end{table}


==> tables/tab_chi2_weighted.tex <==
\begin{table}[t]
        \tiny
        \centering
        \begin{tabular}{lc|c|c|c|c|c|}
                \toprule
       & & \multicolumn{2}{c}{SM} & \multicolumn{2}{c}{$W=8\cdot 10^{-5}$}\\
          \midrule
       Dataset  & $n_{\rm dat}$ & $\chi^2$  & $\chi^2$ (weighted) & $\chi^2$ & $\chi^2$ (weighted) \\
          \midrule
           E866 (NuSea) & 89 & 0.80 & 0.81 & 0.98 & 1.14 \\
           D0  $W$ muon asymmetry & 9 & 2.38 & 2.76 & 3.05  & 3.82\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) central & 46 & 0.81 & 0.82 & 0.82 & 0.82\\
         ATLAS \(W, Z\) 7 TeV (${\cal L}=4.6\,{\rm fb}^{-1}$) forward & 15 & 1.82 & 1.80 & 1.81 & 1.80 \\
%                \midrule
%                ATLAS high-mass DY 7 TeV (${\cal L}=49\,{\rm fb}^{-1}$)& 13 & 0.85  & 0.85 & 0.87 & 0.84 \\
%                ATLAS high-mass DY 2D 8 TeV & 46 & 0.86 & 0.85 & 0.88 & 0.86 \\
%                CMS high-mass DY 2D 7 TeV & 117 & 0.90 & 0.90 & 0.91 & 0.90 \\
%                CMS high-mass DY 8 TeV & 41 & 0.84 & 0.84 & 0.85 & 0.84 \\
%                CMS high-mass DY 13 TeV & 43 & 1.12 & 1.12 &1.13 & 1.13 \\
                \midrule
                HL-LHC NC \(e\)& 16 & 1.98 & 1.79 & 2.21 & 1.83 \\
                HL-LHC NC \(\mu\)& 16 & 1.10 & 1.04 & 1.17 & 1.05\\
                HL-LHC CC \(e\)& 12 & 0.75 & 0.74 & 1.14 & 0.77\\
                HL-LHC CC \(\mu\)& 12 & 0.65 & 0.64 & 1.16 & 0.63  \\
                \midrule
                \textbf{Total} & \textbf{4771} & \textbf{0.97} & -1.41 & \textbf{0.96} &-1.89 \\
                \bottomrule
        \end{tabular}
        \caption{\label{tab:chi2weighted} Values of the \(\chi^2\) per data point  in the baseline and in the $\hat{W}=8\cdot 10^{-5}$ contaminated fit 
        in the regular fit and in a weighted fit in which high-mass Drell-Yan data are given a larger weight according to Eq.~\eqref{eq:wgts}.}
\end{table}
